Automated risk classification of colon biopsies based on semantic segmentation of histopathology images

Artificial Intelligence (AI) can potentially support histopathologists in the diagnosis of a broad spectrum of cancer types. In colorectal cancer (CRC), AI can alleviate the laborious task of characterization and reporting on resected biopsies, including polyps, the numbers of which are increasing as a result of CRC population screening programs, ongoing in many countries all around the globe. Here, we present an approach to address two major challenges in automated assessment of CRC histopathology whole-slide images. First, we present an AI-based method to segment multiple tissue compartments in the H\&E-stained whole-slide image, which provides a different, more perceptible picture of tissue morphology and composition. We test and compare a panel of state-of-the-art loss functions available for segmentation models, and provide indications about their use in histopathology image segmentation, based on the analysis of a) a multi-centric cohort of CRC cases from five medical centers in the Netherlands and Germany, and b) two publicly available datasets on segmentation in CRC. Second, we use the best performing AI model as the basis for a computer-aided diagnosis system (CAD) that classifies colon biopsies into four main categories that are relevant pathologically. We report the performance of this system on an independent cohort of more than 1,000 patients. The results show the potential of such an AI-based system to assist pathologists in diagnosis of CRC in the context of population screening. We have made the segmentation model available for research use on https://grand-challenge.org/algorithms/colon-tissue-segmentation/.

==> Tissue segmentation medical image analsyis/bokhorst19 <==
\begin{thebibliography}{29}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\href}[2]{#2}
\providecommand{\path}[1]{#1}
\providecommand{\DOIprefix}{doi:}
\providecommand{\ArXivprefix}{arXiv:}
\providecommand{\URLprefix}{URL: }
\providecommand{\Pubmedprefix}{pmid:}
\providecommand{\doi}[1]{\href{http://dx.doi.org/#1}{\path{#1}}}
\providecommand{\Pubmed}[1]{\href{pmid:#1}{\path{#1}}}
\providecommand{\bibinfo}[2]{#2}
\ifx\xfnm\relax \def\xfnm[#1]{\unskip,\space#1}\fi
%Type = Inproceedings
\bibitem[{Altun et~al.(2020)Altun, Chlebus, Jacobs, Meine, van Ginneken and
  Hahn}]{altu20}
\bibinfo{author}{Altun, H.C.}, \bibinfo{author}{Chlebus, G.},
  \bibinfo{author}{Jacobs, C.}, \bibinfo{author}{Meine, H.},
  \bibinfo{author}{van Ginneken, B.}, \bibinfo{author}{Hahn, H.K.},
  \bibinfo{year}{2020}.
\newblock \bibinfo{title}{Feasibility of end-to-end trainable two-stage u-net
  for detection of axillary lymph nodes in contrast-enhanced ct based on sparse
  annotations}, in: \bibinfo{booktitle}{Medical Imaging 2020: Computer-Aided
  Diagnosis}, \bibinfo{organization}{International Society for Optics and
  Photonics}. p. \bibinfo{pages}{113141C}.
%Type = Article
\bibitem[{Amid et~al.(2019)Amid, Warmuth, Anil and Koren}]{amid19}
\bibinfo{author}{Amid, E.}, \bibinfo{author}{Warmuth, M.K.},
  \bibinfo{author}{Anil, R.}, \bibinfo{author}{Koren, T.},
  \bibinfo{year}{2019}.
\newblock \bibinfo{title}{Robust bi-tempered logistic loss based on bregman
  divergences}.
\newblock \bibinfo{journal}{arXiv preprint arXiv:1906.03361} .
%Type = Misc
\bibitem[{Antonio et~al.()Antonio, Ahti, Guglielmo, Carl, Partha, Nereo,
  Mariano, Maja, Joakim, Maria, Klara~Miriam, Stefan, Isabelle, Rengaswamy and
  Diama}]{eusc17}
\bibinfo{author}{Antonio, P.}, \bibinfo{author}{Ahti, A.},
  \bibinfo{author}{Guglielmo, R.}, \bibinfo{author}{Carl, o.S.},
  \bibinfo{author}{Partha, B.}, \bibinfo{author}{Nereo, S.},
  \bibinfo{author}{Mariano, T.}, \bibinfo{author}{Maja, P.Z.},
  \bibinfo{author}{Joakim, D.}, \bibinfo{author}{Maria, F.},
  \bibinfo{author}{Klara~Miriam, E.}, \bibinfo{author}{Stefan, L.},
  \bibinfo{author}{Isabelle, S.}, \bibinfo{author}{Rengaswamy, S.},
  \bibinfo{author}{Diama, V.}, .
\newblock \bibinfo{title}{Cancer screening in the european union (2017)}.
\newblock
  \bibinfo{note}{\url{https://ec.europa.eu/health/sites/health/files/major_chronic_diseases/docs/2017_cancerscreening_2ndreportimplementation_en.pdf}}.
%Type = Article
\bibitem[{Ardila et~al.(2019)Ardila, Kiraly, Bharadwaj, Choi, Reicher, Peng,
  Tse, Etemadi, Ye, Corrado et~al.}]{Ardi19}
\bibinfo{author}{Ardila, D.}, \bibinfo{author}{Kiraly, A.P.},
  \bibinfo{author}{Bharadwaj, S.}, \bibinfo{author}{Choi, B.},
  \bibinfo{author}{Reicher, J.J.}, \bibinfo{author}{Peng, L.},
  \bibinfo{author}{Tse, D.}, \bibinfo{author}{Etemadi, M.},
  \bibinfo{author}{Ye, W.}, \bibinfo{author}{Corrado, G.}, et~al.,
  \bibinfo{year}{2019}.
\newblock \bibinfo{title}{End-to-end lung cancer screening with
  three-dimensional deep learning on low-dose chest computed tomography}.
\newblock \bibinfo{journal}{Nature medicine} \bibinfo{volume}{25},
  \bibinfo{pages}{954--961}.
%Type = Article
\bibitem[{de~Bel et~al.(2021)de~Bel, Bokhorst, van~der Laak and
  Litjens}]{bel21}
\bibinfo{author}{de~Bel, T.}, \bibinfo{author}{Bokhorst, J.M.},
  \bibinfo{author}{van~der Laak, J.}, \bibinfo{author}{Litjens, G.},
  \bibinfo{year}{2021}.
\newblock \bibinfo{title}{Residual cyclegan for robust domain transformation of
  histopathological tissue slides}.
\newblock \bibinfo{journal}{Medical Image Analysis} \bibinfo{volume}{70},
  \bibinfo{pages}{102004}.
%Type = Inproceedings
\bibitem[{Berman et~al.(2018a)Berman, Triki and Blaschko}]{berm18a}
\bibinfo{author}{Berman, M.}, \bibinfo{author}{Triki, A.R.},
  \bibinfo{author}{Blaschko, M.B.}, \bibinfo{year}{2018}a.
\newblock \bibinfo{title}{The lov{\'a}sz-softmax loss: A tractable surrogate
  for the optimization of the intersection-over-union measure in neural
  networks}, in: \bibinfo{booktitle}{Proceedings of the IEEE Conference on
  Computer Vision and Pattern Recognition}, pp. \bibinfo{pages}{4413--4421}.
%Type = Inproceedings
\bibitem[{Berman et~al.(2018b)Berman, Triki and Blaschko}]{Berm18b}
\bibinfo{author}{Berman, M.}, \bibinfo{author}{Triki, A.R.},
  \bibinfo{author}{Blaschko, M.B.}, \bibinfo{year}{2018}b.
\newblock \bibinfo{title}{The lov{\'a}sz-softmax loss: A tractable surrogate
  for the optimization of the intersection-over-union measure in neural
  networks}, in: \bibinfo{booktitle}{Proceedings of the IEEE Conference on
  Computer Vision and Pattern Recognition}, pp. \bibinfo{pages}{4413--4421}.
%Type = Article
\bibitem[{Binder et~al.(2019)Binder, Tantaoui, Pati, Catena, Set-Aghayan and
  Gabrani}]{bind19}
\bibinfo{author}{Binder, T.}, \bibinfo{author}{Tantaoui, E.M.},
  \bibinfo{author}{Pati, P.}, \bibinfo{author}{Catena, R.},
  \bibinfo{author}{Set-Aghayan, A.}, \bibinfo{author}{Gabrani, M.},
  \bibinfo{year}{2019}.
\newblock \bibinfo{title}{Multi-organ gland segmentation using deep learning}.
\newblock \bibinfo{journal}{Frontiers in medicine} \bibinfo{volume}{6},
  \bibinfo{pages}{173}.
%Type = Inproceedings
\bibitem[{Bokhorst et~al.(2019)Bokhorst, Pinckaers, van Zwam, Nagetgaal,
  van~der Laak and Ciompi}]{Bokh19}
\bibinfo{author}{Bokhorst, J.M.}, \bibinfo{author}{Pinckaers, H.},
  \bibinfo{author}{van Zwam, P.}, \bibinfo{author}{Nagetgaal, I.},
  \bibinfo{author}{van~der Laak, J.}, \bibinfo{author}{Ciompi, F.},
  \bibinfo{year}{2019}.
\newblock \bibinfo{title}{Learning from sparsely annotated data for semantic
  segmentation in histopathology images}, pp. \bibinfo{pages}{81--94}.
\newblock \URLprefix \url{http://proceedings.mlr.press/v102/bokhorst19a.html}.
%Type = Inproceedings
\bibitem[{Bulten et~al.(2018)Bulten, Hulsbergen-van~de Kaa, van~der Laak,
  Litjens et~al.}]{bult18}
\bibinfo{author}{Bulten, W.}, \bibinfo{author}{Hulsbergen-van~de Kaa, C.A.},
  \bibinfo{author}{van~der Laak, J.}, \bibinfo{author}{Litjens, G.J.}, et~al.,
  \bibinfo{year}{2018}.
\newblock \bibinfo{title}{Automated segmentation of epithelial tissue in
  prostatectomy slides using deep learning}, in: \bibinfo{booktitle}{Medical
  Imaging 2018: Digital Pathology}, \bibinfo{organization}{International
  Society for Optics and Photonics}. p. \bibinfo{pages}{105810S}.
%Type = Article
\bibitem[{Bulten et~al.(2020)Bulten, Pinckaers, van Boven, Vink, de~Bel, van
  Ginneken, van~der Laak, Hulsbergen-van~de Kaa and Litjens}]{bult20}
\bibinfo{author}{Bulten, W.}, \bibinfo{author}{Pinckaers, H.},
  \bibinfo{author}{van Boven, H.}, \bibinfo{author}{Vink, R.},
  \bibinfo{author}{de~Bel, T.}, \bibinfo{author}{van Ginneken, B.},
  \bibinfo{author}{van~der Laak, J.}, \bibinfo{author}{Hulsbergen-van~de Kaa,
  C.}, \bibinfo{author}{Litjens, G.}, \bibinfo{year}{2020}.
\newblock \bibinfo{title}{Automated deep-learning system for gleason grading of
  prostate cancer using biopsies: a diagnostic study}.
\newblock \bibinfo{journal}{The Lancet Oncology} \bibinfo{volume}{21},
  \bibinfo{pages}{233--241}.
%Type = Article
\bibitem[{De~Fauw et~al.(2018)De~Fauw, Ledsam, Romera-Paredes, Nikolov,
  Tomasev, Blackwell, Askham, Glorot, O’Donoghue, Visentin et~al.}]{Fauw18}
\bibinfo{author}{De~Fauw, J.}, \bibinfo{author}{Ledsam, J.R.},
  \bibinfo{author}{Romera-Paredes, B.}, \bibinfo{author}{Nikolov, S.},
  \bibinfo{author}{Tomasev, N.}, \bibinfo{author}{Blackwell, S.},
  \bibinfo{author}{Askham, H.}, \bibinfo{author}{Glorot, X.},
  \bibinfo{author}{O’Donoghue, B.}, \bibinfo{author}{Visentin, D.}, et~al.,
  \bibinfo{year}{2018}.
\newblock \bibinfo{title}{Clinically applicable deep learning for diagnosis and
  referral in retinal disease}.
\newblock \bibinfo{journal}{Nature medicine} \bibinfo{volume}{24},
  \bibinfo{pages}{1342--1350}.
%Type = Article
\bibitem[{Eelbode et~al.(2020)Eelbode, Bertels, Berman, Vandermeulen, Maes,
  Bisschops and Blaschko}]{eelb20}
\bibinfo{author}{Eelbode, T.}, \bibinfo{author}{Bertels, J.},
  \bibinfo{author}{Berman, M.}, \bibinfo{author}{Vandermeulen, D.},
  \bibinfo{author}{Maes, F.}, \bibinfo{author}{Bisschops, R.},
  \bibinfo{author}{Blaschko, M.B.}, \bibinfo{year}{2020}.
\newblock \bibinfo{title}{Optimization for medical image segmentation: theory
  and practice when evaluating with dice score or jaccard index}.
\newblock \bibinfo{journal}{IEEE Transactions on Medical Imaging}
  \bibinfo{volume}{39}, \bibinfo{pages}{3679--3690}.
%Type = Article
\bibitem[{Esteva et~al.(2017)Esteva, Kuprel, Novoa, Ko, Swetter, Blau and
  Thrun}]{Este17}
\bibinfo{author}{Esteva, A.}, \bibinfo{author}{Kuprel, B.},
  \bibinfo{author}{Novoa, R.A.}, \bibinfo{author}{Ko, J.},
  \bibinfo{author}{Swetter, S.M.}, \bibinfo{author}{Blau, H.M.},
  \bibinfo{author}{Thrun, S.}, \bibinfo{year}{2017}.
\newblock \bibinfo{title}{Dermatologist-level classification of skin cancer
  with deep neural networks}.
\newblock \bibinfo{journal}{nature} \bibinfo{volume}{542},
  \bibinfo{pages}{115--118}.
%Type = Article
\bibitem[{Graham et~al.(2019)Graham, Chen, Gamper, Dou, Heng, Snead, Tsang and
  Rajpoot}]{grah19}
\bibinfo{author}{Graham, S.}, \bibinfo{author}{Chen, H.},
  \bibinfo{author}{Gamper, J.}, \bibinfo{author}{Dou, Q.},
  \bibinfo{author}{Heng, P.A.}, \bibinfo{author}{Snead, D.},
  \bibinfo{author}{Tsang, Y.W.}, \bibinfo{author}{Rajpoot, N.},
  \bibinfo{year}{2019}.
\newblock \bibinfo{title}{Mild-net: Minimal information loss dilated network
  for gland instance segmentation in colon histology images}.
\newblock \bibinfo{journal}{Medical image analysis} \bibinfo{volume}{52},
  \bibinfo{pages}{199--211}.
%Type = Inproceedings
\bibitem[{He et~al.(2016)He, Zhang, Ren and Sun}]{he15b}
\bibinfo{author}{He, K.}, \bibinfo{author}{Zhang, X.}, \bibinfo{author}{Ren,
  S.}, \bibinfo{author}{Sun, J.}, \bibinfo{year}{2016}.
\newblock \bibinfo{title}{Deep residual learning for image recognition}, in:
  \bibinfo{booktitle}{Proceedings of the IEEE conference on computer vision and
  pattern recognition}, pp. \bibinfo{pages}{770--778}.
%Type = Article
\bibitem[{Korbar et~al.(2017)Korbar, Olofson, Miraflor, Nicka, Suriawinata,
  Torresani, Suriawinata and Hassanpour}]{korb17}
\bibinfo{author}{Korbar, B.}, \bibinfo{author}{Olofson, A.M.},
  \bibinfo{author}{Miraflor, A.P.}, \bibinfo{author}{Nicka, C.M.},
  \bibinfo{author}{Suriawinata, M.A.}, \bibinfo{author}{Torresani, L.},
  \bibinfo{author}{Suriawinata, A.A.}, \bibinfo{author}{Hassanpour, S.},
  \bibinfo{year}{2017}.
\newblock \bibinfo{title}{Deep learning for classification of colorectal polyps
  on whole-slide images}.
\newblock \bibinfo{journal}{Journal of pathology informatics}
  \bibinfo{volume}{8}.
%Type = Inproceedings
\bibitem[{Lin et~al.(2017)Lin, Goyal, Girshick, He and Doll{\'a}r}]{Lin17a}
\bibinfo{author}{Lin, T.Y.}, \bibinfo{author}{Goyal, P.},
  \bibinfo{author}{Girshick, R.}, \bibinfo{author}{He, K.},
  \bibinfo{author}{Doll{\'a}r, P.}, \bibinfo{year}{2017}.
\newblock \bibinfo{title}{Focal loss for dense object detection}, in:
  \bibinfo{booktitle}{Proceedings of the IEEE international conference on
  computer vision}, pp. \bibinfo{pages}{2980--2988}.
%Type = Inproceedings
\bibitem[{Liu et~al.(2016)Liu, Anguelov, Erhan, Szegedy, Reed, Fu and
  Berg}]{liu16}
\bibinfo{author}{Liu, W.}, \bibinfo{author}{Anguelov, D.},
  \bibinfo{author}{Erhan, D.}, \bibinfo{author}{Szegedy, C.},
  \bibinfo{author}{Reed, S.}, \bibinfo{author}{Fu, C.Y.},
  \bibinfo{author}{Berg, A.C.}, \bibinfo{year}{2016}.
\newblock \bibinfo{title}{Ssd: Single shot multibox detector}, in:
  \bibinfo{booktitle}{European conference on computer vision},
  \bibinfo{organization}{Springer}. pp. \bibinfo{pages}{21--37}.
%Type = Inproceedings
\bibitem[{Long et~al.(2015)Long, Shelhamer and Darrell}]{long15}
\bibinfo{author}{Long, J.}, \bibinfo{author}{Shelhamer, E.},
  \bibinfo{author}{Darrell, T.}, \bibinfo{year}{2015}.
\newblock \bibinfo{title}{Fully convolutional networks for semantic
  segmentation}, in: \bibinfo{booktitle}{Proceedings of the IEEE conference on
  computer vision and pattern recognition}, pp. \bibinfo{pages}{3431--3440}.
%Type = Inproceedings
\bibitem[{Naik et~al.(2008)Naik, Doyle, Agner, Madabhushi, Feldman and
  Tomaszewski}]{naik08}
\bibinfo{author}{Naik, S.}, \bibinfo{author}{Doyle, S.},
  \bibinfo{author}{Agner, S.}, \bibinfo{author}{Madabhushi, A.},
  \bibinfo{author}{Feldman, M.}, \bibinfo{author}{Tomaszewski, J.},
  \bibinfo{year}{2008}.
\newblock \bibinfo{title}{Automated gland and nuclei segmentation for grading
  of prostate and breast cancer histopathology}, in: \bibinfo{booktitle}{2008
  5th IEEE International Symposium on Biomedical Imaging: From Nano to Macro},
  \bibinfo{organization}{IEEE}. pp. \bibinfo{pages}{284--287}.
%Type = Article
\bibitem[{Qin et~al.(2018)Qin, Chen, Zeng, Chai and Wang}]{qin18}
\bibinfo{author}{Qin, P.}, \bibinfo{author}{Chen, J.}, \bibinfo{author}{Zeng,
  J.}, \bibinfo{author}{Chai, R.}, \bibinfo{author}{Wang, L.},
  \bibinfo{year}{2018}.
\newblock \bibinfo{title}{Large-scale tissue histopathology image segmentation
  based on feature pyramid}.
\newblock \bibinfo{journal}{EURASIP Journal on Image and Video Processing}
  \bibinfo{volume}{2018}, \bibinfo{pages}{1--9}.
%Type = Inproceedings
\bibitem[{Rahman and Wang(2016)}]{rahm16}
\bibinfo{author}{Rahman, M.A.}, \bibinfo{author}{Wang, Y.},
  \bibinfo{year}{2016}.
\newblock \bibinfo{title}{Optimizing intersection-over-union in deep neural
  networks for image segmentation}, in: \bibinfo{booktitle}{International
  symposium on visual computing}, \bibinfo{organization}{Springer}. pp.
  \bibinfo{pages}{234--244}.
%Type = Inproceedings
\bibitem[{Redmon and Farhadi(2017)}]{redm17}
\bibinfo{author}{Redmon, J.}, \bibinfo{author}{Farhadi, A.},
  \bibinfo{year}{2017}.
\newblock \bibinfo{title}{Yolo9000: better, faster, stronger}, in:
  \bibinfo{booktitle}{Proceedings of the IEEE conference on computer vision and
  pattern recognition}, pp. \bibinfo{pages}{7263--7271}.
%Type = Inproceedings
\bibitem[{Ronneberger et~al.(2015)Ronneberger, Fischer and Brox}]{ronn15}
\bibinfo{author}{Ronneberger, O.}, \bibinfo{author}{Fischer, P.},
  \bibinfo{author}{Brox, T.}, \bibinfo{year}{2015}.
\newblock \bibinfo{title}{U-net: Convolutional networks for biomedical image
  segmentation}, in: \bibinfo{booktitle}{International Conference on Medical
  image computing and computer-assisted intervention},
  \bibinfo{organization}{Springer}. pp. \bibinfo{pages}{234--241}.
%Type = Article
\bibitem[{Sirinukunwattana et~al.(2017)Sirinukunwattana, Pluim, Chen, Qi, Heng,
  Guo, Wang, Matuszewski, Bruni, Sanchez et~al.}]{siri17}
\bibinfo{author}{Sirinukunwattana, K.}, \bibinfo{author}{Pluim, J.P.},
  \bibinfo{author}{Chen, H.}, \bibinfo{author}{Qi, X.}, \bibinfo{author}{Heng,
  P.A.}, \bibinfo{author}{Guo, Y.B.}, \bibinfo{author}{Wang, L.Y.},
  \bibinfo{author}{Matuszewski, B.J.}, \bibinfo{author}{Bruni, E.},
  \bibinfo{author}{Sanchez, U.}, et~al., \bibinfo{year}{2017}.
\newblock \bibinfo{title}{Gland segmentation in colon histology images: The
  glas challenge contest}.
\newblock \bibinfo{journal}{Medical image analysis} \bibinfo{volume}{35},
  \bibinfo{pages}{489--502}.
%Type = Incollection
\bibitem[{Sudre et~al.(2017)Sudre, Li, Vercauteren, Ourselin and
  Cardoso}]{sudr17}
\bibinfo{author}{Sudre, C.H.}, \bibinfo{author}{Li, W.},
  \bibinfo{author}{Vercauteren, T.}, \bibinfo{author}{Ourselin, S.},
  \bibinfo{author}{Cardoso, M.J.}, \bibinfo{year}{2017}.
\newblock \bibinfo{title}{Generalised dice overlap as a deep learning loss
  function for highly unbalanced segmentations}, in: \bibinfo{booktitle}{Deep
  learning in medical image analysis and multimodal learning for clinical
  decision support}. \bibinfo{publisher}{Springer}, pp.
  \bibinfo{pages}{240--248}.
%Type = Article
\bibitem[{Wulczyn et~al.(2021)Wulczyn, Steiner, Moran, Plass, Reihs, Tan,
  Flament-Auvigne, Brown, Regitnig, Chen et~al.}]{wulc21}
\bibinfo{author}{Wulczyn, E.}, \bibinfo{author}{Steiner, D.F.},
  \bibinfo{author}{Moran, M.}, \bibinfo{author}{Plass, M.},
  \bibinfo{author}{Reihs, R.}, \bibinfo{author}{Tan, F.},
  \bibinfo{author}{Flament-Auvigne, I.}, \bibinfo{author}{Brown, T.},
  \bibinfo{author}{Regitnig, P.}, \bibinfo{author}{Chen, P.H.C.}, et~al.,
  \bibinfo{year}{2021}.
\newblock \bibinfo{title}{Interpretable survival prediction for colorectal
  cancer using deep learning}.
\newblock \bibinfo{journal}{npj Digital Medicine} \bibinfo{volume}{4},
  \bibinfo{pages}{1--13}.
%Type = Article
\bibitem[{Xu et~al.(2020)Xu, Walker, Liang, Tong, Xu, Su and Karsan}]{xu20b}
\bibinfo{author}{Xu, L.}, \bibinfo{author}{Walker, B.}, \bibinfo{author}{Liang,
  P.I.}, \bibinfo{author}{Tong, Y.}, \bibinfo{author}{Xu, C.},
  \bibinfo{author}{Su, Y.C.}, \bibinfo{author}{Karsan, A.},
  \bibinfo{year}{2020}.
\newblock \bibinfo{title}{Colorectal cancer detection based on deep learning}.
\newblock \bibinfo{journal}{Journal of Pathology Informatics}
  \bibinfo{volume}{11}.

\end{thebibliography}


==> bokhorst19 <==
\begin{thebibliography}{29}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\href}[2]{#2}
\providecommand{\path}[1]{#1}
\providecommand{\DOIprefix}{doi:}
\providecommand{\ArXivprefix}{arXiv:}
\providecommand{\URLprefix}{URL: }
\providecommand{\Pubmedprefix}{pmid:}
\providecommand{\doi}[1]{\href{http://dx.doi.org/#1}{\path{#1}}}
\providecommand{\Pubmed}[1]{\href{pmid:#1}{\path{#1}}}
\providecommand{\bibinfo}[2]{#2}
\ifx\xfnm\relax \def\xfnm[#1]{\unskip,\space#1}\fi
%Type = Inproceedings
\bibitem[{Altun et~al.(2020)Altun, Chlebus, Jacobs, Meine, van Ginneken and
  Hahn}]{altu20}
\bibinfo{author}{Altun, H.C.}, \bibinfo{author}{Chlebus, G.},
  \bibinfo{author}{Jacobs, C.}, \bibinfo{author}{Meine, H.},
  \bibinfo{author}{van Ginneken, B.}, \bibinfo{author}{Hahn, H.K.},
  \bibinfo{year}{2020}.
\newblock \bibinfo{title}{Feasibility of end-to-end trainable two-stage u-net
  for detection of axillary lymph nodes in contrast-enhanced ct based on sparse
  annotations}, in: \bibinfo{booktitle}{Medical Imaging 2020: Computer-Aided
  Diagnosis}, \bibinfo{organization}{International Society for Optics and
  Photonics}. p. \bibinfo{pages}{113141C}.
%Type = Article
\bibitem[{Amid et~al.(2019)Amid, Warmuth, Anil and Koren}]{amid19}
\bibinfo{author}{Amid, E.}, \bibinfo{author}{Warmuth, M.K.},
  \bibinfo{author}{Anil, R.}, \bibinfo{author}{Koren, T.},
  \bibinfo{year}{2019}.
\newblock \bibinfo{title}{Robust bi-tempered logistic loss based on bregman
  divergences}.
\newblock \bibinfo{journal}{arXiv preprint arXiv:1906.03361} .
%Type = Misc
\bibitem[{Antonio et~al.()Antonio, Ahti, Guglielmo, Carl, Partha, Nereo,
  Mariano, Maja, Joakim, Maria, Klara~Miriam, Stefan, Isabelle, Rengaswamy and
  Diama}]{eusc17}
\bibinfo{author}{Antonio, P.}, \bibinfo{author}{Ahti, A.},
  \bibinfo{author}{Guglielmo, R.}, \bibinfo{author}{Carl, o.S.},
  \bibinfo{author}{Partha, B.}, \bibinfo{author}{Nereo, S.},
  \bibinfo{author}{Mariano, T.}, \bibinfo{author}{Maja, P.Z.},
  \bibinfo{author}{Joakim, D.}, \bibinfo{author}{Maria, F.},
  \bibinfo{author}{Klara~Miriam, E.}, \bibinfo{author}{Stefan, L.},
  \bibinfo{author}{Isabelle, S.}, \bibinfo{author}{Rengaswamy, S.},
  \bibinfo{author}{Diama, V.}, .
\newblock \bibinfo{title}{Cancer screening in the european union (2017)}.
\newblock
  \bibinfo{note}{\url{https://ec.europa.eu/health/sites/health/files/major_chronic_diseases/docs/2017_cancerscreening_2ndreportimplementation_en.pdf}}.
%Type = Article
\bibitem[{Ardila et~al.(2019)Ardila, Kiraly, Bharadwaj, Choi, Reicher, Peng,
  Tse, Etemadi, Ye, Corrado et~al.}]{Ardi19}
\bibinfo{author}{Ardila, D.}, \bibinfo{author}{Kiraly, A.P.},
  \bibinfo{author}{Bharadwaj, S.}, \bibinfo{author}{Choi, B.},
  \bibinfo{author}{Reicher, J.J.}, \bibinfo{author}{Peng, L.},
  \bibinfo{author}{Tse, D.}, \bibinfo{author}{Etemadi, M.},
  \bibinfo{author}{Ye, W.}, \bibinfo{author}{Corrado, G.}, et~al.,
  \bibinfo{year}{2019}.
\newblock \bibinfo{title}{End-to-end lung cancer screening with
  three-dimensional deep learning on low-dose chest computed tomography}.
\newblock \bibinfo{journal}{Nature medicine} \bibinfo{volume}{25},
  \bibinfo{pages}{954--961}.
%Type = Article
\bibitem[{de~Bel et~al.(2021)de~Bel, Bokhorst, van~der Laak and
  Litjens}]{bel21}
\bibinfo{author}{de~Bel, T.}, \bibinfo{author}{Bokhorst, J.M.},
  \bibinfo{author}{van~der Laak, J.}, \bibinfo{author}{Litjens, G.},
  \bibinfo{year}{2021}.
\newblock \bibinfo{title}{Residual cyclegan for robust domain transformation of
  histopathological tissue slides}.
\newblock \bibinfo{journal}{Medical Image Analysis} \bibinfo{volume}{70},
  \bibinfo{pages}{102004}.
%Type = Inproceedings
\bibitem[{Berman et~al.(2018a)Berman, Triki and Blaschko}]{berm18a}
\bibinfo{author}{Berman, M.}, \bibinfo{author}{Triki, A.R.},
  \bibinfo{author}{Blaschko, M.B.}, \bibinfo{year}{2018}a.
\newblock \bibinfo{title}{The lov{\'a}sz-softmax loss: A tractable surrogate
  for the optimization of the intersection-over-union measure in neural
  networks}, in: \bibinfo{booktitle}{Proceedings of the IEEE Conference on
  Computer Vision and Pattern Recognition}, pp. \bibinfo{pages}{4413--4421}.
%Type = Inproceedings
\bibitem[{Berman et~al.(2018b)Berman, Triki and Blaschko}]{Berm18b}
\bibinfo{author}{Berman, M.}, \bibinfo{author}{Triki, A.R.},
  \bibinfo{author}{Blaschko, M.B.}, \bibinfo{year}{2018}b.
\newblock \bibinfo{title}{The lov{\'a}sz-softmax loss: A tractable surrogate
  for the optimization of the intersection-over-union measure in neural
  networks}, in: \bibinfo{booktitle}{Proceedings of the IEEE Conference on
  Computer Vision and Pattern Recognition}, pp. \bibinfo{pages}{4413--4421}.
%Type = Article
\bibitem[{Binder et~al.(2019)Binder, Tantaoui, Pati, Catena, Set-Aghayan and
  Gabrani}]{bind19}
\bibinfo{author}{Binder, T.}, \bibinfo{author}{Tantaoui, E.M.},
  \bibinfo{author}{Pati, P.}, \bibinfo{author}{Catena, R.},
  \bibinfo{author}{Set-Aghayan, A.}, \bibinfo{author}{Gabrani, M.},
  \bibinfo{year}{2019}.
\newblock \bibinfo{title}{Multi-organ gland segmentation using deep learning}.
\newblock \bibinfo{journal}{Frontiers in medicine} \bibinfo{volume}{6},
  \bibinfo{pages}{173}.
%Type = Inproceedings
\bibitem[{Bokhorst et~al.(2019)Bokhorst, Pinckaers, van Zwam, Nagetgaal,
  van~der Laak and Ciompi}]{Bokh19}
\bibinfo{author}{Bokhorst, J.M.}, \bibinfo{author}{Pinckaers, H.},
  \bibinfo{author}{van Zwam, P.}, \bibinfo{author}{Nagetgaal, I.},
  \bibinfo{author}{van~der Laak, J.}, \bibinfo{author}{Ciompi, F.},
  \bibinfo{year}{2019}.
\newblock \bibinfo{title}{Learning from sparsely annotated data for semantic
  segmentation in histopathology images}, pp. \bibinfo{pages}{81--94}.
\newblock \URLprefix \url{http://proceedings.mlr.press/v102/bokhorst19a.html}.
%Type = Inproceedings
\bibitem[{Bulten et~al.(2018)Bulten, Hulsbergen-van~de Kaa, van~der Laak,
  Litjens et~al.}]{bult18}
\bibinfo{author}{Bulten, W.}, \bibinfo{author}{Hulsbergen-van~de Kaa, C.A.},
  \bibinfo{author}{van~der Laak, J.}, \bibinfo{author}{Litjens, G.J.}, et~al.,
  \bibinfo{year}{2018}.
\newblock \bibinfo{title}{Automated segmentation of epithelial tissue in
  prostatectomy slides using deep learning}, in: \bibinfo{booktitle}{Medical
  Imaging 2018: Digital Pathology}, \bibinfo{organization}{International
  Society for Optics and Photonics}. p. \bibinfo{pages}{105810S}.
%Type = Article
\bibitem[{Bulten et~al.(2020)Bulten, Pinckaers, van Boven, Vink, de~Bel, van
  Ginneken, van~der Laak, Hulsbergen-van~de Kaa and Litjens}]{bult20}
\bibinfo{author}{Bulten, W.}, \bibinfo{author}{Pinckaers, H.},
  \bibinfo{author}{van Boven, H.}, \bibinfo{author}{Vink, R.},
  \bibinfo{author}{de~Bel, T.}, \bibinfo{author}{van Ginneken, B.},
  \bibinfo{author}{van~der Laak, J.}, \bibinfo{author}{Hulsbergen-van~de Kaa,
  C.}, \bibinfo{author}{Litjens, G.}, \bibinfo{year}{2020}.
\newblock \bibinfo{title}{Automated deep-learning system for gleason grading of
  prostate cancer using biopsies: a diagnostic study}.
\newblock \bibinfo{journal}{The Lancet Oncology} \bibinfo{volume}{21},
  \bibinfo{pages}{233--241}.
%Type = Article
\bibitem[{De~Fauw et~al.(2018)De~Fauw, Ledsam, Romera-Paredes, Nikolov,
  Tomasev, Blackwell, Askham, Glorot, O’Donoghue, Visentin et~al.}]{Fauw18}
\bibinfo{author}{De~Fauw, J.}, \bibinfo{author}{Ledsam, J.R.},
  \bibinfo{author}{Romera-Paredes, B.}, \bibinfo{author}{Nikolov, S.},
  \bibinfo{author}{Tomasev, N.}, \bibinfo{author}{Blackwell, S.},
  \bibinfo{author}{Askham, H.}, \bibinfo{author}{Glorot, X.},
  \bibinfo{author}{O’Donoghue, B.}, \bibinfo{author}{Visentin, D.}, et~al.,
  \bibinfo{year}{2018}.
\newblock \bibinfo{title}{Clinically applicable deep learning for diagnosis and
  referral in retinal disease}.
\newblock \bibinfo{journal}{Nature medicine} \bibinfo{volume}{24},
  \bibinfo{pages}{1342--1350}.
%Type = Article
\bibitem[{Eelbode et~al.(2020)Eelbode, Bertels, Berman, Vandermeulen, Maes,
  Bisschops and Blaschko}]{eelb20}
\bibinfo{author}{Eelbode, T.}, \bibinfo{author}{Bertels, J.},
  \bibinfo{author}{Berman, M.}, \bibinfo{author}{Vandermeulen, D.},
  \bibinfo{author}{Maes, F.}, \bibinfo{author}{Bisschops, R.},
  \bibinfo{author}{Blaschko, M.B.}, \bibinfo{year}{2020}.
\newblock \bibinfo{title}{Optimization for medical image segmentation: theory
  and practice when evaluating with dice score or jaccard index}.
\newblock \bibinfo{journal}{IEEE Transactions on Medical Imaging}
  \bibinfo{volume}{39}, \bibinfo{pages}{3679--3690}.
%Type = Article
\bibitem[{Esteva et~al.(2017)Esteva, Kuprel, Novoa, Ko, Swetter, Blau and
  Thrun}]{Este17}
\bibinfo{author}{Esteva, A.}, \bibinfo{author}{Kuprel, B.},
  \bibinfo{author}{Novoa, R.A.}, \bibinfo{author}{Ko, J.},
  \bibinfo{author}{Swetter, S.M.}, \bibinfo{author}{Blau, H.M.},
  \bibinfo{author}{Thrun, S.}, \bibinfo{year}{2017}.
\newblock \bibinfo{title}{Dermatologist-level classification of skin cancer
  with deep neural networks}.
\newblock \bibinfo{journal}{nature} \bibinfo{volume}{542},
  \bibinfo{pages}{115--118}.
%Type = Article
\bibitem[{Graham et~al.(2019)Graham, Chen, Gamper, Dou, Heng, Snead, Tsang and
  Rajpoot}]{grah19}
\bibinfo{author}{Graham, S.}, \bibinfo{author}{Chen, H.},
  \bibinfo{author}{Gamper, J.}, \bibinfo{author}{Dou, Q.},
  \bibinfo{author}{Heng, P.A.}, \bibinfo{author}{Snead, D.},
  \bibinfo{author}{Tsang, Y.W.}, \bibinfo{author}{Rajpoot, N.},
  \bibinfo{year}{2019}.
\newblock \bibinfo{title}{Mild-net: Minimal information loss dilated network
  for gland instance segmentation in colon histology images}.
\newblock \bibinfo{journal}{Medical image analysis} \bibinfo{volume}{52},
  \bibinfo{pages}{199--211}.
%Type = Inproceedings
\bibitem[{He et~al.(2016)He, Zhang, Ren and Sun}]{he15b}
\bibinfo{author}{He, K.}, \bibinfo{author}{Zhang, X.}, \bibinfo{author}{Ren,
  S.}, \bibinfo{author}{Sun, J.}, \bibinfo{year}{2016}.
\newblock \bibinfo{title}{Deep residual learning for image recognition}, in:
  \bibinfo{booktitle}{Proceedings of the IEEE conference on computer vision and
  pattern recognition}, pp. \bibinfo{pages}{770--778}.
%Type = Article
\bibitem[{Korbar et~al.(2017)Korbar, Olofson, Miraflor, Nicka, Suriawinata,
  Torresani, Suriawinata and Hassanpour}]{korb17}
\bibinfo{author}{Korbar, B.}, \bibinfo{author}{Olofson, A.M.},
  \bibinfo{author}{Miraflor, A.P.}, \bibinfo{author}{Nicka, C.M.},
  \bibinfo{author}{Suriawinata, M.A.}, \bibinfo{author}{Torresani, L.},
  \bibinfo{author}{Suriawinata, A.A.}, \bibinfo{author}{Hassanpour, S.},
  \bibinfo{year}{2017}.
\newblock \bibinfo{title}{Deep learning for classification of colorectal polyps
  on whole-slide images}.
\newblock \bibinfo{journal}{Journal of pathology informatics}
  \bibinfo{volume}{8}.
%Type = Inproceedings
\bibitem[{Lin et~al.(2017)Lin, Goyal, Girshick, He and Doll{\'a}r}]{Lin17a}
\bibinfo{author}{Lin, T.Y.}, \bibinfo{author}{Goyal, P.},
  \bibinfo{author}{Girshick, R.}, \bibinfo{author}{He, K.},
  \bibinfo{author}{Doll{\'a}r, P.}, \bibinfo{year}{2017}.
\newblock \bibinfo{title}{Focal loss for dense object detection}, in:
  \bibinfo{booktitle}{Proceedings of the IEEE international conference on
  computer vision}, pp. \bibinfo{pages}{2980--2988}.
%Type = Inproceedings
\bibitem[{Liu et~al.(2016)Liu, Anguelov, Erhan, Szegedy, Reed, Fu and
  Berg}]{liu16}
\bibinfo{author}{Liu, W.}, \bibinfo{author}{Anguelov, D.},
  \bibinfo{author}{Erhan, D.}, \bibinfo{author}{Szegedy, C.},
  \bibinfo{author}{Reed, S.}, \bibinfo{author}{Fu, C.Y.},
  \bibinfo{author}{Berg, A.C.}, \bibinfo{year}{2016}.
\newblock \bibinfo{title}{Ssd: Single shot multibox detector}, in:
  \bibinfo{booktitle}{European conference on computer vision},
  \bibinfo{organization}{Springer}. pp. \bibinfo{pages}{21--37}.
%Type = Inproceedings
\bibitem[{Long et~al.(2015)Long, Shelhamer and Darrell}]{long15}
\bibinfo{author}{Long, J.}, \bibinfo{author}{Shelhamer, E.},
  \bibinfo{author}{Darrell, T.}, \bibinfo{year}{2015}.
\newblock \bibinfo{title}{Fully convolutional networks for semantic
  segmentation}, in: \bibinfo{booktitle}{Proceedings of the IEEE conference on
  computer vision and pattern recognition}, pp. \bibinfo{pages}{3431--3440}.
%Type = Inproceedings
\bibitem[{Naik et~al.(2008)Naik, Doyle, Agner, Madabhushi, Feldman and
  Tomaszewski}]{naik08}
\bibinfo{author}{Naik, S.}, \bibinfo{author}{Doyle, S.},
  \bibinfo{author}{Agner, S.}, \bibinfo{author}{Madabhushi, A.},
  \bibinfo{author}{Feldman, M.}, \bibinfo{author}{Tomaszewski, J.},
  \bibinfo{year}{2008}.
\newblock \bibinfo{title}{Automated gland and nuclei segmentation for grading
  of prostate and breast cancer histopathology}, in: \bibinfo{booktitle}{2008
  5th IEEE International Symposium on Biomedical Imaging: From Nano to Macro},
  \bibinfo{organization}{IEEE}. pp. \bibinfo{pages}{284--287}.
%Type = Article
\bibitem[{Qin et~al.(2018)Qin, Chen, Zeng, Chai and Wang}]{qin18}
\bibinfo{author}{Qin, P.}, \bibinfo{author}{Chen, J.}, \bibinfo{author}{Zeng,
  J.}, \bibinfo{author}{Chai, R.}, \bibinfo{author}{Wang, L.},
  \bibinfo{year}{2018}.
\newblock \bibinfo{title}{Large-scale tissue histopathology image segmentation
  based on feature pyramid}.
\newblock \bibinfo{journal}{EURASIP Journal on Image and Video Processing}
  \bibinfo{volume}{2018}, \bibinfo{pages}{1--9}.
%Type = Inproceedings
\bibitem[{Rahman and Wang(2016)}]{rahm16}
\bibinfo{author}{Rahman, M.A.}, \bibinfo{author}{Wang, Y.},
  \bibinfo{year}{2016}.
\newblock \bibinfo{title}{Optimizing intersection-over-union in deep neural
  networks for image segmentation}, in: \bibinfo{booktitle}{International
  symposium on visual computing}, \bibinfo{organization}{Springer}. pp.
  \bibinfo{pages}{234--244}.
%Type = Inproceedings
\bibitem[{Redmon and Farhadi(2017)}]{redm17}
\bibinfo{author}{Redmon, J.}, \bibinfo{author}{Farhadi, A.},
  \bibinfo{year}{2017}.
\newblock \bibinfo{title}{Yolo9000: better, faster, stronger}, in:
  \bibinfo{booktitle}{Proceedings of the IEEE conference on computer vision and
  pattern recognition}, pp. \bibinfo{pages}{7263--7271}.
%Type = Inproceedings
\bibitem[{Ronneberger et~al.(2015)Ronneberger, Fischer and Brox}]{ronn15}
\bibinfo{author}{Ronneberger, O.}, \bibinfo{author}{Fischer, P.},
  \bibinfo{author}{Brox, T.}, \bibinfo{year}{2015}.
\newblock \bibinfo{title}{U-net: Convolutional networks for biomedical image
  segmentation}, in: \bibinfo{booktitle}{International Conference on Medical
  image computing and computer-assisted intervention},
  \bibinfo{organization}{Springer}. pp. \bibinfo{pages}{234--241}.
%Type = Article
\bibitem[{Sirinukunwattana et~al.(2017)Sirinukunwattana, Pluim, Chen, Qi, Heng,
  Guo, Wang, Matuszewski, Bruni, Sanchez et~al.}]{siri17}
\bibinfo{author}{Sirinukunwattana, K.}, \bibinfo{author}{Pluim, J.P.},
  \bibinfo{author}{Chen, H.}, \bibinfo{author}{Qi, X.}, \bibinfo{author}{Heng,
  P.A.}, \bibinfo{author}{Guo, Y.B.}, \bibinfo{author}{Wang, L.Y.},
  \bibinfo{author}{Matuszewski, B.J.}, \bibinfo{author}{Bruni, E.},
  \bibinfo{author}{Sanchez, U.}, et~al., \bibinfo{year}{2017}.
\newblock \bibinfo{title}{Gland segmentation in colon histology images: The
  glas challenge contest}.
\newblock \bibinfo{journal}{Medical image analysis} \bibinfo{volume}{35},
  \bibinfo{pages}{489--502}.
%Type = Incollection
\bibitem[{Sudre et~al.(2017)Sudre, Li, Vercauteren, Ourselin and
  Cardoso}]{sudr17}
\bibinfo{author}{Sudre, C.H.}, \bibinfo{author}{Li, W.},
  \bibinfo{author}{Vercauteren, T.}, \bibinfo{author}{Ourselin, S.},
  \bibinfo{author}{Cardoso, M.J.}, \bibinfo{year}{2017}.
\newblock \bibinfo{title}{Generalised dice overlap as a deep learning loss
  function for highly unbalanced segmentations}, in: \bibinfo{booktitle}{Deep
  learning in medical image analysis and multimodal learning for clinical
  decision support}. \bibinfo{publisher}{Springer}, pp.
  \bibinfo{pages}{240--248}.
%Type = Article
\bibitem[{Wulczyn et~al.(2021)Wulczyn, Steiner, Moran, Plass, Reihs, Tan,
  Flament-Auvigne, Brown, Regitnig, Chen et~al.}]{wulc21}
\bibinfo{author}{Wulczyn, E.}, \bibinfo{author}{Steiner, D.F.},
  \bibinfo{author}{Moran, M.}, \bibinfo{author}{Plass, M.},
  \bibinfo{author}{Reihs, R.}, \bibinfo{author}{Tan, F.},
  \bibinfo{author}{Flament-Auvigne, I.}, \bibinfo{author}{Brown, T.},
  \bibinfo{author}{Regitnig, P.}, \bibinfo{author}{Chen, P.H.C.}, et~al.,
  \bibinfo{year}{2021}.
\newblock \bibinfo{title}{Interpretable survival prediction for colorectal
  cancer using deep learning}.
\newblock \bibinfo{journal}{npj Digital Medicine} \bibinfo{volume}{4},
  \bibinfo{pages}{1--13}.
%Type = Article
\bibitem[{Xu et~al.(2020)Xu, Walker, Liang, Tong, Xu, Su and Karsan}]{xu20b}
\bibinfo{author}{Xu, L.}, \bibinfo{author}{Walker, B.}, \bibinfo{author}{Liang,
  P.I.}, \bibinfo{author}{Tong, Y.}, \bibinfo{author}{Xu, C.},
  \bibinfo{author}{Su, Y.C.}, \bibinfo{author}{Karsan, A.},
  \bibinfo{year}{2020}.
\newblock \bibinfo{title}{Colorectal cancer detection based on deep learning}.
\newblock \bibinfo{journal}{Journal of Pathology Informatics}
  \bibinfo{volume}{11}.

\end{thebibliography}

